Adaptive Bandit Convex Optimization with Heterogeneous Curvature

We consider the problem of adversarial bandit convex optimization, that is, online learning over a sequence of arbitrary convex loss functions with only one function evaluation for each of them. While all previous works assume known and homogeneous curvature on these loss functions, we study a heterogeneous setting where each function has its own curvature that is only revealed after the learner makes a decision. We develop an efficient algorithm that is able to adapt to the curvature on the fly. Specifically, our algorithm not only recovers or \emph{even improves} existing results for several homogeneous settings, but also leads to surprising results for some heterogeneous settings -- for example, while Hazan and Levy (2014) showed that $\widetilde{O}(d^{3/2}\sqrt{T})$ regret is achievable for a sequence of $T$ smooth and strongly convex $d$-dimensional functions, our algorithm reveals that the same is achievable even if $T^{3/4}$ of them are not strongly convex, and sometimes even if a constant fraction of them are not strongly convex. Our approach is inspired by the framework of Bartlett et al. (2007) who studied a similar heterogeneous setting but with stronger gradient feedback. Extending their framework to the bandit feedback setting requires novel ideas such as lifting the feasible domain and using a logarithmically homogeneous self-concordant barrier regularizer.

==> conclusion.tex <==
\section{Conclusion and Future Work}\label{sec: conclusion}

In this work, we consider the problem of BCO where at each round, the curvature information of the loss function is revealed after the decision is made by the learner. While previous works design different algorithms to achieve different regret guarantees when the curvature of the loss functions are different, we design a single novel algorithm with a combination of FTRL with self-concordant barrier regularizer and adaptive learning rate tuning, which achieves the matching regret bounds \emph{without} knowing what the environment is. One future work is that when the curvature information is not correct in some rounds, whether we can design an algorithm that is robust to the possible incorrect curvature information. Another possible but more challenging direction is to design a more efficient algorithm such that $\otil(\sqrt{T})$ regret bound can be achieved for general bandit convex optimization problem. %Furthermore, \citep{COLT'21:efficient-BCO} shows that when the loss function is quadratic, the hessian of the loss function can be well-approximated by using only the observed function value. Howeve Another open direction is whether this curvature information can be approximated under other function classes 
